Learning Graph Models for Retrosynthesis Prediction

Retrosynthesis prediction is a fundamental problem in organic synthesis, where the task is to identify precursor molecules that can be used to synthesize a target molecule. A key consideration in building neural models for this task is aligning model design with strategies adopted by chemists. Building on this viewpoint, this paper introduces a graph-based approach that capitalizes on the idea that the graph topology of precursor molecules is largely unaltered during a chemical reaction. The model first predicts the set of graph edits transforming the target into incomplete molecules called synthons. Next, the model learns to expand synthons into complete molecules by attaching relevant leaving groups. This decomposition simplifies the architecture, making its predictions more interpretable, and also amenable to manual correction. Our model achieves a top-1 accuracy of $53.7\%$, outperforming previous template-free and semi-template-based methods.

==> checklist.tex <==
\newpage
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our work is relevant to scientific disciplines aiming to automate chemical synthesis. Our proposed method has a simplified architecture, that is transparent and allows for manual correction. However, chemical synthesis is a challenging endeavor with gaps between computational and experimental predictions. Furthermore, we make no assumptions regarding the yield of reactions, which can be a limiting factor in chemical synthesis. While potential misuse can never be ruled out, our presented method promises positive societal and scientific impact.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide code, datasets and installation instructions via an external URL.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The dataset splits are described in Appendix~\ref{app:dataset_splits}, hyperparameter tuning described in Appendix~\ref{app:hyperparams}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
	\answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We report the types of resources used as well as the total computation time in Appendix~\ref{app:computing}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{The dataset is provided by \citep{dai2019retrosynthesis} under the MIT License}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide the canonicalized dataset along with our code.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> graph_retro/introduction.tex <==
\section{Introduction} \label{sec:intro}

{\em Retrosynthesis prediction}, first formalized by E.J. Corey \citep{corey1991logic}, is a fundamental problem in organic synthesis that attempts to identify a series of chemical transformations for synthesizing a target molecule. In the single-step formulation, the task is to identify a set of reactant molecules given a target. The problem is challenging as the space of possible transformations is vast, and requires the skill of experienced chemists. Since the 1960s, retrosynthesis prediction has seen assistance from modern computing techniques \citep{corey1969computer}, with a recent surge in machine learning methods \citep{chen2020learning,  coley2017computer, dai2019retrosynthesis, zheng2019predicting}.

Existing machine learning methods for retrosynthesis prediction fall into template-based \citep{coley2017computer, dai2019retrosynthesis, segler2017neural} and template-free approaches \citep{chen2020learning, zheng2019predicting}. Template-based methods match the target molecule against a large set of templates, which are molecular subgraph patterns that highlight changes during a chemical reaction. Despite their interpretability, these methods suffer from poor generalization to new and rare reactions. Template-free methods bypass templates by learning a direct mapping from the SMILES representations \citep{weininger1988smiles} of the product to reactants. Despite their greater generalization potential, these methods generate reactant SMILES character by character, failing to utilize the largely conserved substructures in a chemical reaction. 

A chemical reaction satisfies two \emph{fundamental} properties:
\begin{enumerate*}[label=(\roman*.)]
    \item the product atoms are always a subset of the reactant atoms\footnote{ignoring impurities}, and
    \item the molecular graph topology is largely unaltered from products to reactants
\end{enumerate*}. For example, in the standard retrosynthesis dataset, only 6.3\% of the atoms in the product undergo any change in connectivity. Our approach is motivated by the hypothesis that utilizing subgraphs within the product to generate reactants can significantly improve the performance and generalization ability of retrosynthesis models. 

Our template-free approach called \textsc{GraphRetro} generates reactants in two stages:
\begin{enumerate*}[label=(\roman*.)]
    \item deriving intermediate molecules called synthons from the product molecule, and
    \item expanding synthons into reactants by adding specific functionalities called leaving groups
\end{enumerate*}. For deriving synthons, we utilize the rarity of new bond formations to predict a score for existing bonds and atoms instead of each atom pair. This reduces the prediction complexity from $O(N^2)$ to $O(N)$. Furthermore, we incorporate global dependencies into our prediction input by using convolutional layers. For completing synthons into reactants, we select leaving groups from a precomputed vocabulary. The vocabulary is constructed during preprocessing by extracting subgraphs that differ between a synthon and the corresponding reactant, and has a 99.7\% coverage on the test set.

We evaluate \textsc{GraphRetro} on the benchmark USPTO-50k dataset and a subset of the same dataset that consists of rare reactions. On the USPTO-50k dataset, \textsc{GrapRetro} achieves 64.2\% top-1 accuracy without the knowledge of reaction class, outperforming the state-of-the-art method by a margin of 11.7\%. On the rare reaction subset, \textsc{GraphRetro} achieves 31.5\% top-1 accuracy, with a 4\% margin over the state-of-the-art method.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.02\textwidth]{figures/introduction/overview.pdf}
    \caption[Proposed retrosynthesis workflow]{\textbf{Overview of Our Approach}. \textbf{a}. \textbf{Edit Prediction}. We train a model to learn a distribution over possible graph edits. In this case, the correct edit corresponds to breaking the bond marked in red. Applying this edit produces two synthons. \textbf{b}. \textbf{Synthon Completion}. Another model is trained to pick candidate leaving groups (blue) for each synthon from a discrete vocabulary, which are then attached to produce the final reactants.}
    \label{fig:overview}
\end{figure}


==> misc.tex <==
\section{Experiments}
\label{sec:experiments}

\paragraph{Data} We evaluate the \textsc{GraphRetro} model on the widely used benchmark dataset USPTO-50k \citep{schneider2016s}, which contains 50k atom-mapped reactions across 10 reaction classes. Following \citep{liu2017retrosynthetic, coley2017prediction}, we partition the dataset into a 80\%/10\%/10\% train/development/test split. For the transfer learning experiments, we extract a rare reaction subset of USPTO-50k (see Appendix~\ref{app:rare-reactions}), with \textasciitilde3900 train reactions and 500 reactions in development and test sets. 

\paragraph{Baseline Models} We compare \textsc{GraphRetro} to five baselines. \textsc{LV-Transformer} \citep{chen2020learning} extends the Transformer architecture with a latent variable to improve diversity of suggested reactants. \textsc{SCROP} \citep{zheng2019predicting} uses an additional Transformer to correct the syntax of candidates generated from the first one. \textsc{Retrosim} \cite{coley2017computer} uses molecular similarities to precedent reactions for template ranking. \textsc{NeuralSym} \citep{segler2017neural} learns a conditional distribution over templates given a molecule. The state-of-the-art method, \textsc{GLN} \citep{dai2019retrosynthesis} models the joint distribution of templates and reactants using logic variables. Results of \textsc{NeuralSym} are taken from \cite{dai2019retrosynthesis}.

\paragraph{Evaluation Metrics} Similar to prior work \citep{dai2019retrosynthesis, liu2017retrosynthetic}, we use the top-$n$ exact match accuracy as our evaluation metric, for $n = 1, 3, 5, 10, 20 \text{ and } 50$. The accuracy is computed by matching canonical SMILES strings of predicted reactants with those of ground truth reactants. For the benchmarks, we evaluate the top-$n$ accuracy with and without the knowledge of reaction class. For the latter, the reaction class is added as an additional one-hot vector to atom features. For transfer learning, we evaluate the top-$n$ accuracy for $n = 1, 3, 5 \text{and} 10$, for the setting where the reaction class is unknown.

\subsection{Overall Performance} \label{subsec:pred-perform}
As shown in Table~\ref{tab:overall}, when the reaction class is unknown, our \emph{shared} and \emph{separate} configurations outperform \textsc{GLN} by 11.6\% and 11.2\% in top-1 accuracy, respectively. Similar improvements are achieved for larger $n$, with \textasciitilde85\% of the true precursors in the top-5 choices. Barring \textsc{GLN}, \textsc{GraphRetro}’s top-5 and top-10 accuracies are higher than the top-50 accuracy of other baseline models. When the reaction class is known, \textsc{Retrosim} and \textsc{GLN} restrict template sets corresponding to the reaction class, thus improving performance. Both of our model configurations outperform the other models till $n = 5$.

\begin{table}[]
    \caption{Top-$n$ exact match accuracy. (S) denotes Single-Edit and (M) denotes Multiple Edit}
    \label{tab:overall}
    \vspace{5pt}
    \centering
    \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & 
    \multicolumn{6}{c}{\textbf{Top-$n$ Accuracy (\%)}} \\\cline{2-7}
    & {1} & {3} & {5} & {10} & {20} & {50} \\
    \midrule
    \multicolumn{6}{c}{{Reaction class known}} \\
    \midrule
    \textsc{Retrosim} \citep{coley2017computer}& 52.9	& 73.8 & 81.2 & 88.1 & 91.8 & 92.9 \\
    \textsc{NeuralSym} \citep{segler2017neural}& 55.3 & 76 & 81.4 & 85.1 & 86.5 & 86.9 \\
    \textsc{GLN} \citep{dai2019retrosynthesis} & 63.2 & 77.5 & 83.4 & \cellcolor{blue!15}89.1 & \cellcolor{blue!15}92.1 & \cellcolor{blue!15}93.2 \\
    \textsc{SCROP} \citep{zheng2019predicting}& 59 & 74.8 & 78.1 & 81.1 & - & - \\
    $\mathrm{\textsc{GraphRetro}}^*$ (\emph{shared}) & 67.2 & 82.5 & 85.7 & 87.2 & 87.5 & 87.2\\
    $\mathrm{\textsc{GraphRetro}}^*$ (\emph{separate}) & \cellcolor{blue!15}67.7 &  \cellcolor{blue!15}83.7 & \cellcolor{blue!15}86.6 & 87.9 & 88.1 & 87.9  \\
    \midrule
    \multicolumn{6}{c}{{Reaction class unknown}} \\
    \midrule
    \textsc{Retrosim} \citep{coley2017computer} & 37.3 & 54.7 & 63.3 & 74.1 & 82 & 85.3 \\
    \textsc{NeuralSym} \citep{segler2017neural} & 44.4 & 65.3 & 72.4 & 78.9 & 82.2 & 83.1 \\
    \textsc{GLN} \citep{dai2019retrosynthesis} & 52.6 & 68 & 75.1 & 83.1 & \cellcolor{blue!15}88.5 & \cellcolor{blue!15}92.1 \\
    \textsc{SCROP} \citep{zheng2019predicting} & 43.7 & 60.0 & 65.2 & 68.7 & - & - \\
    \textsc{LV-Transformer} \cite{chen2020learning} & 40.5 & 65.1 & 72.8 & 79.4 & - & - \\
    $\mathrm{\textsc{GraphRetro}(S)}^*$ (\emph{shared}) & \cellcolor{blue!15}64.2 & 80 & 83 & 84.6 & 84.8 & 84.1 \\
    $\mathrm{\textsc{GraphRetro}(S)}^*$ (\emph{separate}) & 63.8 & \cellcolor{blue!15}80.9 & \cellcolor{blue!15}84.5 & \cellcolor{blue!15}86.4 & 87.1 & 87.2 \\
    \bottomrule
    \end{tabular}
\end{table}


\subsection{Individual Module Performance (WIP)} \label{subsec: indi-perform}
As shown in Table~\ref{tab:overall}, when the reaction class is unknown, our \emph{shared} and \emph{separate} configurations outperform \textsc{GLN} by 11.6\% and 11.2\% in top-1 accuracy, respectively. Similar improvements are achieved for larger $n$, with \textasciitilde85\% of the true precursors in the top-5 choices. Barring \textsc{GLN}, \textsc{GraphRetro}’s top-5 and top-10 accuracies are higher than the top-50 accuracy of other baseline models. When the reaction class is known, \textsc{Retrosim} and \textsc{GLN} restrict template sets corresponding to the reaction class, thus improving performance. Both of our model configurations outperform the other models till $n = 5$.

\begin{table*}[h]
\caption{Performance of individual modules}
    \label{tab:ind-perform}
    \vspace{5pt}
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lcccclcccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & 
    \multicolumn{4}{c}{\textbf{Top-$n$ Accuracy (\%)}} &
    \multirow{2}{*}{\textbf{Model}} &  \multicolumn{4}{c}{\textbf{Top-$n$ Accuracy (\%)}} \\\cline{2-5}\cline{7-10}
    & {1} & {3} & {5} & {10} & & {1} & {3} & {5} & {10} \\
    \midrule
    
    \textsc{Retrosim} & 52.9& 73.8 & 81.2 & 88.1 & \textsc{Retrosim} & 37.3 & 54.7 & 63.3 & 74.1 \\
    \textsc{NeuralSym} & 55.3 & 76 & 81.4 & 85.1 & \textsc{NeuralSym} & 44.4 & 65.3 & 72.4 & 78.9 \\
    \textsc{GLN}  & 63.2 & 77.5 & 83.4 & \cellcolor{blue!15}89.1 & \textsc{GLN} & 52.6 & 68 & 75.1 & 83.1\\
    \textsc{SCROP} & 59 & 74.8 & 78.1 & 81.1 & \textsc{SCROP} & 43.7 & 60.0 & 65.2 & 68.7 \\
    & & & & & \textsc{LV-Transformer} & 40.5 & 65.1 & 72.8 & 79.4\\
    $\mathrm{\textsc{GraphRetro}}$ (sh) & 67.2 & 82.5 & 85.7 & 87.2 & $\mathrm{\textsc{GraphRetro}}$ (sh) & \cellcolor{blue!15}64.2 & 80 & 83 & 84.6\\
    $\mathrm{\textsc{GraphRetro}}$ (se) & \cellcolor{blue!15}67.7 &  \cellcolor{blue!15}83.7 & \cellcolor{blue!15}86.6 & 87.9 & $\mathrm{\textsc{GraphRetro}}$ (se) & 63.8 & \cellcolor{blue!15}80.9 & \cellcolor{blue!15}84.5 & \cellcolor{blue!15}86.4 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}

\subsection{Transfer Learning (WIP)} \label{subsec:transfer-learn}
As shown in Table~\ref{tab:overall}, when the reaction class is unknown, our \emph{shared} and \emph{separate} configurations outperform \textsc{GLN} by 11.6\% and 11.2\% in top-1 accuracy, respectively. Similar improvements are achieved for larger $n$, with \textasciitilde85\% of the true precursors in the top-5 choices. Barring \textsc{GLN}, \textsc{GraphRetro}’s top-5 and top-10 accuracies are higher than the top-50 accuracy of other baseline models. When the reaction class is known, \textsc{Retrosim} and \textsc{GLN} restrict template sets corresponding to the reaction class, thus improving performance. Both of our model configurations outperform the other models till $n = 5$.

\begin{table*}[h]
\caption{Transfer Learning}
    \label{tab:transfer-learning}
    \vspace{5pt}
    \centering  
    
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lcccclcccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & 
    \multicolumn{4}{c}{\textbf{Top-$n$ Accuracy (\%)}} &
    \multirow{2}{*}{\textbf{Model}} &  \multicolumn{4}{c}{\textbf{Top-$n$ Accuracy (\%)}} \\\cline{2-5}\cline{7-10}
    & {1} & {3} & {5} & {10} & & {1} & {3} & {5} & {10} \\
    \midrule
    
    \textsc{Retrosim} & 52.9& 73.8 & 81.2 & 88.1 & \textsc{Retrosim} & 37.3 & 54.7 & 63.3 & 74.1 \\
    \textsc{NeuralSym} & 55.3 & 76 & 81.4 & 85.1 & \textsc{NeuralSym} & 44.4 & 65.3 & 72.4 & 78.9 \\
    \textsc{GLN}  & 63.2 & 77.5 & 83.4 & \cellcolor{blue!15}89.1 & \textsc{GLN} & 52.6 & 68 & 75.1 & 83.1\\
    \textsc{SCROP} & 59 & 74.8 & 78.1 & 81.1 & \textsc{SCROP} & 43.7 & 60.0 & 65.2 & 68.7 \\
    & & & & & \textsc{LV-Transformer} & 40.5 & 65.1 & 72.8 & 79.4\\
    $\mathrm{\textsc{GraphRetro}}$ (sh) & 67.2 & 82.5 & 85.7 & 87.2 & $\mathrm{\textsc{GraphRetro}}$ (sh) & \cellcolor{blue!15}64.2 & 80 & 83 & 84.6\\
    $\mathrm{\textsc{GraphRetro}}$ (se) & \cellcolor{blue!15}67.7 &  \cellcolor{blue!15}83.7 & \cellcolor{blue!15}86.6 & 87.9 & $\mathrm{\textsc{GraphRetro}}$ (se) & 63.8 & \cellcolor{blue!15}80.9 & \cellcolor{blue!15}84.5 & \cellcolor{blue!15}86.4 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}

\subsection{Example Predictions (WIP) } \label{subsec:example-predictions} Figure~\ref{fig:correct-example} shows an example where the edit and leaving groups are identified correctly. In Figure~\ref{fig:incorrect-example}, the correct edit is identified but the predicted leaving groups are incorrect. In the training set, leaving groups attaching to the carbonyl carbon (C=O) are small (e.g. -OH, -NH$_2$, halides). The true leaving group in this example, however, is large. \textsc{GraphRetro} is unable to reason about this and predicts the small leaving group -I.

\begin{figure}[H]
\centering
\begin{subfigure}{0.5\columnwidth}
 \centering
  \includegraphics[width=0.75\linewidth]{figures/discussion/correct-nei-2.pdf}
  \label{fig:neia}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}
 \centering
  \includegraphics[width=0.75\linewidth]{figures/discussion/correct-nei-1.pdf}
  \label{fig:neib}
\end{subfigure}
\caption[Example of successful edit predictions after using local neighborhood information]{Example of successful edit predictions (\emph{green}) after incorporating local neighborhood interactions. Incorrect edits predicted previously are shown in \emph{red}. The model identifies a multiple ring aromatic system (\emph{left}) and bond polarities (\emph{right}).}
\label{fig:Edit prediction with NA}
\end{figure}

\begin{figure}[]
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/discussion/correct-example.pdf}
  \caption{Successful Prediction}
  \label{fig:correct-example}
\end{subfigure}
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/discussion/incorrect-example.pdf}
  \caption{Unsuccessful Prediction}
  \label{fig:incorrect-example}
\end{subfigure}
\caption[Example predictions]{Example predictions. The true edit and incorrect edit (if any) are highlighted in green and red respectively. The true and predicted leaving groups are highlighted in yellow.} 
\label{fig:example-predictions}
\end{figure}

% Figure~\ref{fig:correct-example} illustrates a correctly predicted example by the model. Figure~\ref{fig:incorrect-example} offers an interesting insight into the model's reasoning. Here, the edit prediction module identifies the edit correctly, but the synthon completion module predicts the leaving groups incorrectly. Upon further examination, it appears as if the synthon completion module reversed the predictions for the synthons. In the training set, leaving groups that attach to the carbonyl carbon (C=O) are small (e.g. -OH, -NH$_2$, halides). However in this case, the true leaving group is larger which is harder for the model to reason about, resulting in the leaving group -I as its prediction. %Similarly, aromatic rings occur with large groups or other aromatic rings in their vicinity, resulting in the prediction of a larger leaving group, instead of the -Br group.


==> rare_reactions.tex <==
\section{Rare Reactions}
\label{sec:rare_reactions}

Natural product synthesis presents a unique challenge for retrosynthesis through a combination of low resource learning, complex target molecules and rare or unseen chemical transformations. Pretraining and transfer learning present attractive options for training deep models for this task. As datasets for natural product synthesis are not available, we construct a rare reaction subset from our training set (details in Appendix~\ref{app:transfer_learning}) to study transfer learning. We evaluate two approaches:

\subsection{Direct Transfer}
\label{subsec:pretrain_model}
This is akin to the general transfer learning setup where the model is first trained on a larger dataset and then finetuned on the smaller dataset. We apply this strategy to both the \emph{shared} and \emph{separate} configurations of \textsc{GraphRetro}.

\subsection{Contrastive Learning of Reactions (RCL)}
\label{subsec:pretrain_encoder}
We propose a contrastive learning strategy to pretrain the encoder that learns representations of products and reactants reflective of their reaction chemistry. Our method is based on the premise that a product-synthon-reactant tuple for a given reaction are closer to each other in the reaction space than arbitrary combinations from different reactions. The components of our setup include:

\textbf{Graph encoder} $f(\cdot)$ that computes a graph representation given a graph $\mathcal{G}$. The setup is agnostic of the choice of graph encoder. We use the message passing network (MPN) as our encoder.
    
\textbf{Reaction space projection} $g(\cdot)$ that maps the graph representation to the reaction space. We use a MLP with one hidden layer to obtain $\mathbf{h}_\mathcal{G} = \mathbf{W_2} \left(\mathrm{\tau}\left(\mathbf{W_1}\mathbf{c}_{\mathcal{G}} + b_1\right)\right)$. This projection network is necessary as the ``closeness'' between products, synthons and reactants is enforced in the reaction space, not in the representation space. The contrastive loss, thus, is applied to corresponding projections of product, synthon and reactant graph representations.

For every reaction $R_c$, we define two contrastive prediction tasks:

\begin{itemize}
    \item Given $\mathcal{G}_p$ and a set $\{\mathcal{G}_{p'}\}$ which contains a connected component $\mathcal{G}_{s_{c}}$, the \emph{product-synthon} prediction task aims to identify $\mathcal{G}_{s_{c}}$ in $\{\mathcal{G}_{{p}'}\}$. This is repeated for every component $c \leq C$.

    \item Given a set $\{\mathcal{G}_{s'}\}$ and a positive pair of examples $\mathcal{G}_{s_{c}}, \mathcal{G}_{r_{c}}$ \emph{synthon-reactant} contrastive prediction task aims to identify $\mathcal{G}_{r_{c}}$ in $\{\mathcal{G}_{s'}\}$ given $\mathcal{G}_{s_{c}}$.
\end{itemize}

We sample a random minibatch of $N$ reactions, and use the other $N-1$ reactions as negative examples. Given vectors $\mathbf{h}_i$, $\mathbf{h}_j$, we define the similarity $s_{ij}$ as their dot product $s_{ij}= \mathbf{h}_i^{T} \mathbf{h}_j$. The similarity function accommodates both unnormalized and normalized vectors. 

\paragraph{Training} The model is trained to minimize the following loss function: 

\begin{align}
    \mathcal{L\left(\mathcal{T}\right)} & = \sum_{\mathcal{B} \in \mathcal{T}} {\sum_{k \in \{p, s\}}{\sum_{(\mathcal{G}_k, \{\mathcal{G}_{{k}'}\}) \in \mathcal{B}}}{\mathcal{L}^{(k, k')}}} \\
    \mathcal{L}^{(k, k')} & = -\sum_{\mathcal{G}_j \in \{\mathcal{G}_{{k}'}\}}\mathrm{log} \hspace{1pt}\frac{\mathrm{exp(}s_{kj} \hspace{2pt}/ \hspace{2pt}\mathrm{\theta})}{\sum_{j'}{\mathrm{exp(}s_{kj'} \hspace{2pt}/ \hspace{2pt} \mathrm{\theta})}}
\end{align}

where $\mathcal{B}$ indicates the minibatch, $\mathrm{\theta}$ denotes the temperature parameter and $(\mathcal{G}_k, \{\mathcal{G}_{{k}'}\})$ denote the positive - negative example pairs constructed for the two contrastive prediction tasks.
